A Simple Electrostatic Model for the Hard-Sphere Solute Component of Nonpolar Solvation

We propose a new model for estimating the free energy of forming a molecular cavity in a solvent, by assuming this energy is dominated by the electrostatic energy associated with creating the static (interface) potential inside the cavity. The new model approximates the cavity-formation energy as that of a shell capacitor: the inner, solute-shaped conductor is held at the static potential, and the outer conductor (at the first solvation shell) is held at zero potential. Compared to cavity energies computed using free-energy pertubation with explicit-solvent molecular dynamics, the new model exhibits surprising accuracy (Mobley test set, RMSE 0.45 kcal/mol). Combined with a modified continuum model for solute-solvent van der Waals interactions, the total nonpolar model has RMSE of 0.55 kcal/mol on this test set, which is remarkable because the two terms largely cancel. The overall nonpolar model has a small number of physically meaningful parameters and compares favorably to other published models of nonpolar solvation. Finally, when the proposed nonpolar model is combined with our solvation-layer interface condition (SLIC) continuum electrostatic model, which includes asymmetric solvation-shell response, we predict solvation free energies with an RMS error of 1.35 kcal/mol relative to experiment, comparable to the RMS error of explicit-solvent FEP (1.26 kcal/mol). Moreover, all parameters in our model have a clear physical meaning, and employing reasonable temperature dependencies yields remarkable correlation with solvation entropies.

==> Supplementary_material/suppmethods.tex <==

%
\begin{figure}[!h]
\centering
\includegraphics[width=0.3\textwidth]{capacitor.pdf}
\caption{Capacitor model of a solute.}
\label{fig:capacitor}
\end{figure}

Figure \ref{fig:capacitor} is a representation of an uncharged solute immersed in a solvent, with a Stern layer between them.
The interface between the solute and Stern layer is called the solvent-excluded surface (SES), whereas the solvent-accessible surface (SAS) is one water radius away ($\sim 1.4$\AA), in the limit between the Stern layer and the solvent. 
In this model, we place surface charge densities at the SES ($\sigma_{\text{SES}}$) and SAS ($\sigma_{\text{SAS}}$) to reproduce the electrostatic potential distribution seen in an uncharged solute, and compute the energy from this setup.

The electrostatic potential in the Stern layer is induced by the surface charge distributions as follows
%

In this case, as the electrostatic potential is constant in the solute and solvent, there is no need to consider the apparent surface charge from the jump in dielectric constant (see Supplementary Material).

We know the potential just inside the SES is $\phi_\text{static}$, whereas the potential just outside the SAS must be zero.
Then, considering that the potential is continuous across dielectric interfaces and surface charges, we can evaluate Equation \eqref{eq:surface_charge} on the SES and SAS, to get
%
%\begin{align}\label{eq:surface_charge_eval}
%\phi(\mathbf{r}_\text{SES}) = \phi_\text{static} &= \oint_\text{SES} \frac{\sigma_\text{SES}(\mathbf{r}')}{4\pi \epsilon_\text{Stern}|\mathbf{r}_\text{SES}- \mathbf{r}'|} \text{d}\mathbf{r}' + \oint_\text{SAS} \frac{\sigma_\text{SAS}(\mathbf{r}')}{4\pi \epsilon_\text{Stern}|\mathbf{r}_\text{SES}- \mathbf{r}'|} \text{d}\mathbf{r}' \nonumber \\
%\phi(\mathbf{r}_\text{SAS}) = 0 &= \oint_\text{SES} \frac{\sigma_\text{SES}(\mathbf{r}')}{4\pi \epsilon_\text{Stern}|\mathbf{r}_\text{SAS}- \mathbf{r}'|} \text{d}\mathbf{r}' + \oint_\text{SAS} \frac{\sigma_\text{SAS}(\mathbf{r}')}{4\pi \epsilon_\text{Stern}|\mathbf{r}_\text{SAS}- \mathbf{r}'|} \text{d}\mathbf{r}',
%\end{align}
%
%which can be written in matrix form as
%
\begin{equation}\label{eq:matrix}
\left[
\begin{array}{c c}
V_\text{SES} & V_\text{SES}\\
V_\text{SAS} & V_\text{SAS}
\end{array}
\right]
\left[
\begin{array}{c}
\sigma_\text{SES}\\
\sigma_\text{SAS}
\end{array}
\right]
=
\epsilon_\text{Stern}\left[
\begin{array}{c}
\phi_\text{static}\\
0 
\end{array}
\right]
\end{equation}
%
Here, $V_{\Gamma_1}(\psi_{\Gamma_2}) = \oint_{\Gamma_2} \frac{\psi(\mathbf{r}')}{4\pi|\mathbf{r}_{\Gamma_1} - \mathbf{r}'|}\text{d}\mathbf{r}'$ is the single-layer potential of the distribution $\psi$ on $\Gamma_2$, evaluated on a point located in $\Gamma_1$.
%
%\begin{equation}\label{eq:single_layer}
%V_{\Gamma_1}(\psi_{\Gamma_2}) = \oint_{\Gamma_2} \frac{\psi(\mathbf{r}')}{4\pi|\mathbf{r}_{\Gamma_1} - \mathbf{r}'|}\text{d}\mathbf{r}'.
%\end{equation}

We solve for $\sigma_\text{SES}$ and $\sigma_\text{SAS}$ in Equation \eqref{eq:matrix} with a boundary element method (BEM) using the \texttt{bempp} library \cite{SmigajETal2015}.
The BEM generates a numerical version of Equation \eqref{eq:matrix} starting from a surface discretized in flat triangular panels (obtained using \texttt{msms} \cite{SannerOlsonSpehner1995}), and solves for $\sigma_\text{SES}$ and $\sigma_\text{SAS}$. 
With \texttt{bempp}, we assume a piecewise constant distribution of $\sigma_\text{SAS}$ and $\sigma_\text{SES}$ on the molecular surface, and use a Galerkin approach to generate a matrix which we solve with a GMRES algorithm.

Having the surface charge distributions, and considering that the potential on the SAS is zero, we can compute the energy with 
%
\begin{equation}\label{eq:energy}
\Delta G_\text{cav} = \oint_\text{SES} \phi_\text{static}\sigma_\text{SES}(\mathbf{r})\text{d}\mathbf{r}
\end{equation}

By using continuum electrostatic theory, the solvent degrees of freedom are averaged out, making Equation \eqref{eq:energy} a free energy calculation \cite{RouxSimonson1999}.
In particular, $\Delta G_\text{cav}$ is the electrostatic contribution to the difference in Gibbs free energy between the solvent in bulk state (no free energy) and with a cavity, which equals the reversible work required to generate the void where the solute will fit. 
%This should not be confused with the so-called solvent reorganization energy \cite{YuKarplus1988,Lazaridis2000,GallicchioKuboLevy2000}, which refers to the binding energy of a single solvent molecule as it is surrounded by the rest of the solvent.
%That solvent reorganization energy contributes to the internal energy, and not the free energy directly.

%%%%%\subsection{A surface integral approach for $\Delta G_\text{vdw}$}
Levy {\it et al.} \cite{LevyZhangGallicchioFelts2003} used a continuum description to compute the energy from solute-solvent dispersion interactions based on the integral of the Lennard-Jones potential over the solvent. Later, Bardhan {\it et al.}\cite{BardhanETal2005} used the divergence theorem to reformulate it as
%
\begin{equation}\label{eq:vdw_energy}
\Delta G_\text{disp} = \sum_i \oint_\text{SAS} \rho_w \frac{\partial}{\partial \mathbf{n}}\left( \frac{A_i}{90|\mathbf{r} - \mathbf{r}_i|^{10}}
- \frac{B_i}{12|\mathbf{r} - \mathbf{r}_i|^4}\right) \text{d}\mathbf{r}  
\end{equation}
%
%\begin{equation}\label{eq:vdw_volume}
%\Delta G_\text{vdw} = \sum_i \int_\text{solvent} \rho_w \left(\frac{A_i}{|\mathbf{r}-\mathbf{r}_i|^{12}} - \frac{B_i}{|\mathbf{r}-\mathbf{r}_i|^{6}}\right) \text{d}\mathbf{r}
%\end{equation}
%
where $\rho_w$ is the solvent number density, $A_i$ and $B_i$ are the Lennard-Jones parameters for atom $i$, and the sum is over the solute's atoms. Also, the unit vector $\mathbf{n}$ points away from the SAS. 
%In the work by Bardhan {\it et al.} \cite{BardhanETal2005}, the authors use the divergence theorem to represent Equation \eqref{eq:vdw_volume} as a surface integral, which gives
%
%
%where $\mathbf{n}$ is a unit vector normal to the SAS, pointing into the solvent.
The formulation in Equation \eqref{eq:vdw_energy} is very convenient to our model, as it only requires a mesh over the SAS, which we already have from the calculation of $\Delta G_\text{cav}$.

It is well known that the water density increases near interfaces CITE. 
We account for this fact by considering a thin layer that is one water molecule radius thick ($1.4$\AA) beyond the SAS with a higher density, in our case, set to $1.8\rho_w$.
This, however, can be seen as a fitting parameter for the dispersion energy.


%-------------------
%The nonpolar component of the solvation energy is usually decomposed into $\Delta G_\text{cav} + \Delta G_\text{disp}$, the sum of the energy required to generate the cavity plus the energy from the solute-solvent dispersion interaction, respectively.\cite{GallicchioZhangLevy2002} This decomposition is discussed in the Supplementary Material and sketched in Figure S1. Here, we detail the models used for $\Delta G_\text{cav}$ and $\Delta G_\text{disp}$. 


==> discussion.tex <==
%\subsection{Accuracy of the implicit solvent model for $\Delta G_\text{nonpolar}$}

%It is important to note that the repulsive potential ($\phi_\text{rep}$ in Equation \eqref{eq:wca}) used to compute $\Delta G_\text{cav}$ with molecular dynamics includes a Lennard-Jones component, which is substracted out from $\phi_\text{att}$.
%In Equation \eqref{eq:vdw_energy}, all of the Lennard-Jones potential is accounted in $\Delta G_\text{vdw}$, and not in $\Delta G_\text{cav}$. 
%This makes $\Delta G_\text{cav}$ and $\Delta G_\text{vdw}$ computed with an explicit solvent, in principle, slightly different to our implicit solvent model.
%Regarless of this discrepancy, we see an exceptional correlation. 
%Moreover, the small $\Delta G_\text{nonpolar}$ is the sum between larger positive $\Delta G_\text{cav}$ and negative $\Delta G_\text{disp}$, making it a challenge to obtain good correlation.
%Even though $\rho_p$ degrades to $0.88$, the correlation is still remarkable, which is further supported by the MUE and RMSD being below $0.5$kcal/mol.


%To obtain optimal results with SASA models, the surface tension ($\gamma$) needs to be molecule dependent. 
%For example, in Michael {\it et al.} \cite{MichaelETal2017} the authors considered four different surface tension coefficients for ions and alkane, polar, and aromatic molecules, ranging from $\gamma=-50$ to $\gamma=20$ kcal/mol/\AA. 
%Considering that the cavity is uncharged, an appropriate description should not be a function of any aspect that is unique to the solute, besides its geometry, indicating that the SASA model is not giving a complete physical picture. 

%\begin{itemize}
%\item We get better correlation than the best model around
%\item Model is based on fitting parameters that have more robust physical interpretation 
%\item We use one set of parameters for all solutes (DISA model has different parameters for polar molecules and alkanes).
%\item Some elements that are consistently poorly correlated: triple bonds (\#), Br, C3
%\item What are the implications here?
%    \begin{itemize}
%    \item Role of electrostatics in the cavity formation? 
%    \item Relation between electrostatics and hydrophobic effect?
%    \item Relation between electrostatic potential and surface tension?
%    \item How does temperature affect? 
%    \end{itemize}
%\end{itemize}


==> other_points.tex <==
\begin{itemize}
\item Our model is semi-empirical, as it assumes that $\Delta G_\text{cav}$ is equal to the free energy stored in the solvation layer (when it is just one of multiple components), and then models that single component using a simple mean-field theory. It seems possible that the capacitor-charging model may be written as some combination of steps involving discharging and charging the solvent atoms. {\bf Chris:} I'm not that sure here. What other components of free energy are there around? Even though there are some 'empirical' things in our model ($\epsilon$ and $\phi_\text{static}$), I would claim it is pretty much theory based. What do you think about this?
\item the best physical picture we have, description cut from the theory section:  electrostatic contribution to the difference in Gibbs free energy between having a bulk-like solvent structure around the solute cavity (zero mean potential in the solute), and the actual solvation-layer structure which creates $\phi_\text{static}$, which equals the reversible work required to generate the void where the solute will fit.
\item The electrostatic free energy density in the bulk solvent is zero, and likewise inside the solute (basically). 
\end{itemize}

References we want to make sure to cite or at least check
\begin{itemize}
\item Sulea09 (jp8061477) SAMPL-1 found a systematic deviation when using continuum dispersion integrals like ours, but they did not break it down (perhaps did not have access to that specific solvation contribution in their data?)
\item Genheden10 has an interesting nonpolar model for PCM (refs 16 and 17) which works on this one example they study, but presume have to look at refs 16 and 17 for more
\item Knight11 and Brooks, from abstract ``more sophisticated nonpolar models are... likely necessary to more effectively represent
  the underlying physics of solvation and take the quality of hydration free energies estimated from implicit solvent models to the next level.''
\item Chen12 is a Nathan Baker paper -- worth comparing to their results
\item Beglov and Roux, certainly ~\cite{BeglovRoux1995} but perhaps also their HNC papers (per Nathan's point, go look at all 3)
\item \cite{BohincETal2012,BohincBossaMay2017} I haven't read these!
\item ConwayBockris51 Dielectric constant in diffuse and double layers~\cite{ConwayBockrisAmmar1951}
\item \cite{LakeMcCullagh2017} i haven't read this
\item recent Aluru papers ~\cite{MashayakAluru2017,MashayakAluru2018}
\item \cite{RingeOberhoferReuter2017} Matt and I talked with these guys in Pisa
\item \cite{Setny2015,SetnyZacharias2010} i haven't read these by Piotr Setny and Martin Zacharias
\item recent Matyushov dielectric constant near interface~\cite{DinpajoohMatyushov2016}
\item Lazaridis 2000 big paper, it's been a long time~\cite{Lazaridis2000}
\item \cite{AshbaughKalerPaulaitis1999} Ashbaugh99 i don't remember reading this with Paulaitis
\item Floris89 Tomasi early continuum integral for dispersion interactions \cite{FlorisTomasi1989}
\item Gallicchio00, classic big paper \cite{GallicchioKuboLevy2000}
\item Gallicchio02 novel nonpolar hydration free energy ~\cite{GallicchioZhangLevy2002}
\item Chandler papers: \cite{HuangChandler2000,HuangChandler2000b,HuangChandler2002,HuangGeisslerChandler2001,LumChandlerWeeks1999}
\item Hummer information theory model ~\cite{HummerETal1996}
\item Michael et al test of different nonpolar models \cite{MichaelETal2017}
\item Guo-Wei Wei on LJ potential to solvation~\cite{NguyenWei2017} not yet convinced we need to cite this
\item Chandler paper with Amish Patel who is at UPenn \cite{VarillyPatelChandler2011}
\item Wei paper on breaking poplar nonpolar division~\cite{WangWangWuWei2018} i haven't read this
\item separating cavity and dispersion terms \cite{Zacharias2003}
\item WagonerBaker PNAS ~\cite{WagonerBaker2006}
\end{itemize}


